Zero-Shot Multi-Label Topic Inference with Sentence Encoders

Sentence encoders have indeed been shown to achieve superior performances for many downstream text-mining tasks and, thus, claimed to be fairly general. Inspired by this, we performed a detailed study on how to leverage these sentence encoders for the "zero-shot topic inference" task, where the topics are defined/provided by the users in real-time. Extensive experiments on seven different datasets demonstrate that Sentence-BERT demonstrates superior generality compared to other encoders, while Universal Sentence Encoder can be preferred when efficiency is a top priority.

==> Dataset.tex <==
\section{Data-sets}\label{sec:data-sets}
 In our experiments we mainly focused on working 2 different type of data-sets. (A) Large data-sets with higher number articles for categorization and relatively longer text (News and Medical-Blog, collected from the web), and (B) Smaller data-sets which contain fewer articles for categorization and relatively shorter in length (Amazon data-sets: Apex, Canon, Creative, Nikon, Nokia, collected from~\cite{karmaker2016generative}).




\subsection{Large Data-sets}
A collection of publicly available online news and medical-blog articles were crawled from the web to create our large data-sets. Each article is already labeled with one or more ground-truth topics and we stored them as JSON objects. Some statistics about these data-sets are summarised in table~\ref{table:Dataset}.

\subsection{Small Data-sets}
The small data-sets are originally a set of 5 different online product reviews. Unlike large data-sets, the product reviews are shorter in length and contains more topics compared to the above 2 data-sets.


%For an example, a review which speaks about concept "Focus" and "Mode" from the Nikon review dataset is "\textit{would be really good if they have given an option to stop this autofocussing}". 


\begin{table}[htb!]
\begin{adjustbox}{width=\linewidth,center}
\centering
\begin{tabular}{ c c c c}
\hline 
 {\textbf{Data-set}}  & {\textbf{Articles}}  & {\textbf{Unique Topics}}  & {\textbf{Topics/article}}\\
\hline
Medical & 2066 & 18 & 1.128  \\
News  & 8940 & 12 & 0.805   \\
Apex  & 839 & 23 & 0.781 \\
Canon  & 642  & 24  & 1.069\\
Creative & 1811 &  21 & 0.956 \\
Nikon  & 380 & 20 & 1.039 \\
Nokia & 587 &  23 & 1.058\\
\hline
\end{tabular}
\end{adjustbox}
\caption{\label{table:Dataset} Statistics on Large and Small data-sets }
\vspace{-5mm}
\end{table}

\subsection{Challenges of Zero-shot Topic Categorization}
A closer look into into the data-sets revealed that they are comprised of articles with varying length and each article is a complex representation of various topics, entities and events and most of the topics are not explicitly mentioned in the article and are thus ``implicit'' topics. The difference between the two can be further clarified through an example. We consider a topic as explicit if the topic name/phrase is explicitly mentioned in the article text. For example, the following sentence is from an article related to topic \textit{\textbf{Corona virus}}, \textbf{\textit{``Americans should feel much better about the topic virus coming under control''}}, which mentions the topic \textit{\textbf{Corona virus}} explicitly in the text body. Whereas, for implicit cases, the topic name is not directly mentioned in the article text, rather the topic is somewhat implied. For example, the following sentence is taken from an article annotated with the topic \textit{\textbf{Women's Health}},\textbf{\textit{ "Studies question: ban on alcohol during pregnancy."}} Here, the text does not contain the phrase \textit{\textbf{Women's Health}}, yet a human can easily relate it to the same topic. %We consider these cases as implicit mentions on the target concept. Based on the above observation, we conclude that simply checking the concept name in the text will not yield a high quality automatic annotation.
Recognizing implicit topics is an arduous job. Probing our data-sets, we ascertained significant portions of the data contains these implicit concepts, hence their accurate identification, is indeed very challenging, specially without any supervision.

==> Zero-shot ARR - arXiv/Dataset.tex <==
\section{Data-sets}\label{sec:data-sets}
 In our experiments we mainly focused on working 2 different type of data-sets. (A) Large data-sets with higher number articles for categorization and relatively longer text (News and Medical-Blog, collected from the web), and (B) Smaller data-sets which contain fewer articles for categorization and relatively shorter in length (Amazon data-sets: Apex, Canon, Creative, Nikon, Nokia, collected from~\cite{karmaker2016generative}).




\subsection{Large Data-sets}
A collection of publicly available online news and medical-blog articles were crawled from the web to create our large data-sets. Each article is already labeled with one or more ground-truth topics and we stored them as JSON objects. Some statistics about these data-sets are summarised in table~\ref{table:Dataset}.

\subsection{Small Data-sets}
The small data-sets are originally a set of 5 different online product reviews. Unlike large data-sets, the product reviews are shorter in length and contains more topics compared to the above 2 data-sets.


%For an example, a review which speaks about concept "Focus" and "Mode" from the Nikon review dataset is "\textit{would be really good if they have given an option to stop this autofocussing}". 


\begin{table}[htb!]
\begin{adjustbox}{width=\linewidth,center}
\centering
\begin{tabular}{ c c c c}
\hline 
 {\textbf{Data-set}}  & {\textbf{Articles}}  & {\textbf{Unique Topics}}  & {\textbf{Topics/article}}\\
\hline
Medical & 2066 & 18 & 1.128  \\
News  & 8940 & 12 & 0.805   \\
Apex  & 839 & 23 & 0.781 \\
Canon  & 642  & 24  & 1.069\\
Creative & 1811 &  21 & 0.956 \\
Nikon  & 380 & 20 & 1.039 \\
Nokia & 587 &  23 & 1.058\\
\hline
\end{tabular}
\end{adjustbox}
\caption{\label{table:Dataset} Statistics on Large and Small data-sets }
\vspace{-5mm}
\end{table}

\subsection{Challenges of Zero-shot Topic Categorization}
A closer look into into the data-sets revealed that they are comprised of articles with varying length and each article is a complex representation of various topics, entities and events and most of the topics are not explicitly mentioned in the article and are thus ``implicit'' topics. The difference between the two can be further clarified through an example. We consider a topic as explicit if the topic name/phrase is explicitly mentioned in the article text. For example, the following sentence is from an article related to topic \textit{\textbf{Corona virus}}, \textbf{\textit{``Americans should feel much better about the topic virus coming under control''}}, which mentions the topic \textit{\textbf{Corona virus}} explicitly in the text body. Whereas, for implicit cases, the topic name is not directly mentioned in the article text, rather the topic is somewhat implied. For example, the following sentence is taken from an article annotated with the topic \textit{\textbf{Women's Health}},\textbf{\textit{ "Studies question: ban on alcohol during pregnancy."}} Here, the text does not contain the phrase \textit{\textbf{Women's Health}}, yet a human can easily relate it to the same topic. %We consider these cases as implicit mentions on the target concept. Based on the above observation, we conclude that simply checking the concept name in the text will not yield a high quality automatic annotation.
Recognizing implicit topics is an arduous job. Probing our data-sets, we ascertained significant portions of the data contains these implicit concepts, hence their accurate identification, is indeed very challenging, specially without any supervision.
